AT-2FF: Adaptive Type-2 Fuzzy Filter for De-noising Images Corrupted with Salt-and-Pepper

Noise is inevitably common in digital images, leading to visual image deterioration. Therefore, a suitable filtering method is required to lessen the noise while preserving the image features (edges, corners, etc.). This paper presents the efficient type-2 fuzzy weighted mean filter with an adaptive threshold to remove the SAP noise. The present filter has two primary steps: The first stage categorizes images as lightly, medium, and heavily corrupted based on an adaptive threshold by comparing the M-ALD of processed pixels with the upper and lower MF of the type-2 fuzzy identifier. The second stage eliminates corrupted pixels by computing the appropriate weight using GMF with the mean and variance of the uncorrupted pixels in the filter window. Simulation results vividly show that the obtained denoised images preserve image features, i.e., edges, corners, and other sharp structures, compared with different filtering methods.

==> acro_list.tex <==
\begin{acronym}[LMF] % Give the longest label here so that the list is nicely aligned
\acro{SAP}{Salt and Pepper}
\acro{MF}{Membership Function}
\acro{PSNR}{Peak Signal-to-Noise Ratio}
\acro{LMF}{Lower Membership Function}
\acro{UMF}{Upper Membership Function}
\acro{BD}{Bonferroni-Dunn}
\acro{CD}{Critical Difference}
\end{acronym}
